On-Device Federated Continual Learning on RISC-V-based Ultra-Low-Power SoC for Intelligent Nano-Drone Swarms

RISC-V-based architectures are paving the way for efficient On-Device Learning (ODL) in smart edge devices. When applied across multiple nodes, ODL enables the creation of intelligent sensor networks that preserve data privacy. However, developing ODL-capable, battery-operated embedded platforms presents significant challenges due to constrained computational resources and limited device lifetime, besides intrinsic learning issues such as catastrophic forgetting. We face these challenges by proposing a regularization-based On-Device Federated Continual Learning algorithm tailored for multiple nano-drones performing face recognition tasks. We demonstrate our approach on a RISC-V-based 10-core ultra-low-power SoC, optimizing the ODL computational requirements. We improve the classification accuracy by 24% over naive fine-tuning, requiring 178 ms per local epoch and 10.5 s per global epoch, demonstrating the effectiveness of the architecture for this task.

==> srcs/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We presented an \gls{odfcl} methodology embodied on the RISC-V-based GAP9 \gls{mcu}, demonstrating 24\% accuracy improvements over naive finetuning on a face recognition task distributed over three intelligent sensor nodes.
We demonstrated that on-device \gls{cil} can be achieved in only \qty{10.5}{\second} per learning epoch with memory costs of tens of \qty{}{\kilo \byte}, suitable for nano-\glspl{uav}.
